The Effect of Data Augmentation on Classification of Atrial Fibrillation in Short Single-Lead ECG Signals Using Deep Neural Networks

Cardiovascular diseases are the most common cause of mortality worldwide. Detection of atrial fibrillation (AF) in the asymptomatic stage can help prevent strokes. It also improves clinical decision making through the delivery of suitable treatment such as, anticoagulant therapy, in a timely manner. The clinical significance of such early detection of AF in electrocardiogram (ECG) signals has inspired numerous studies in recent years, of which many aim to solve this task by leveraging machine learning algorithms. ECG datasets containing AF samples, however, usually suffer from severe class imbalance, which if unaccounted for, affects the performance of classification algorithms. Data augmentation is a popular solution to tackle this problem. In this study, we investigate the impact of various data augmentation algorithms, e.g., oversampling, Gaussian Mixture Models (GMMs) and Generative Adversarial Networks (GANs), on solving the class imbalance problem. These algorithms are quantitatively and qualitatively evaluated, compared and discussed in detail. The results show that deep learning-based AF signal classification methods benefit more from data augmentation using GANs and GMMs, than oversampling. Furthermore, the GAN results in circa $3\%$ better AF classification accuracy in average while performing comparably to the GMM in terms of f1-score.

==> 20_literature_review.tex <==
\section{Literature Review}
\begin{comment}
% introduction on the traditional machine learning pipeline
The core of almost all traditional machine learning-based data classification pipelines consists of three main processing blocks, namely data pre-processing, feature extraction (data description) and classification~\cite[Chap.~1]{bishop}. 
Data can be noisy or {\color{black}{scaled on a space with high variance}}, it can contain highly imbalanced classes or the data dimensions may be highly correlated and contain high redundancy. All of the aforementioned sample scenarios are harmful for a classifier and need attention. In data pre-processing block, the main goal is to make the data ready to be fed to the pipeline. Data denoising, data scaling and data augmentation are the popular measures that are undertaken in the data pre-processing block. In the next block, feature extraction provides a better and more appropriate representation of data so that the classes are better separable. Traditionally, the features are handcrafted, meaning that experts define functions (also called descriptors) that transform the data under study to a more representative space. These functions are highly domain-specific. A handful of highly popular descriptors in computer vision which has shown good performance are scale invariant feature transform (SIFT), speeded-up robust features (SURF), binary partition tree (BPT), fast Fourier transform (FFT), wavelet transform, histogram of oriented gradients (HOG), entropy, etc.~\cite{kumar2014survey}. Finally, the classifier is in charge of separating the data into its respective classes by predicting appropriate labels for each sample. The most famous traditional classifiers that can separate data in a nonlinear way are support vector machine (SVM)~\cite{cortes1995support} and random forest (RF)~\cite{breiman2001random}. 

% traditional and non-deep methods
In the literature for electrocardiogram (ECG) signal classification, there are many works that adopt the traditional machine learning pipeline and used handcrafted features and reported well-performing models and accurate results. In the process of feature engineering, cardiological expert knowledge was taken advantage of to calculate representative and distinctive features. These approaches can be categorized into two groups, namely atrial activity and ventricular activity-based analyses. For AF ECG signal classification, the atrial activity-based approaches rely on detecting the presence of F-wave instead of the P-peak~\cite{alcaraz2006wavelet}, ~\cite{du2014novel}, ~\cite{garcia2016application}, ~\cite{ladavich2015rate}, ~\cite{purerfellner2014p}, ~\cite{rodenas2015wavelet}. On the other hand, the ventricular activity-based approaches are based on anomaly detection in the RR intervals in QRS complexes in ECG signals~\cite{alcaraz2010optimal}, ~\cite{carrara2015heart}, ~\cite{demazumder2013dynamic}, ~\cite{huang2010novel}, ~\cite{lake2010accurate}, ~\cite{linker2016accurate}, ~\cite{park2009atrial}, ~\cite{sarkar2008detector}, ~\cite{tateno2001automatic}. Recent studies tried to aggregate these two approaches, i.e. by fusing both the global features extracted from the whole ECG and from the ones computed from the QRS complex, and could improved the detection rate even further.
The traditional non-linear classifiers such as SVM were exploited for the classification tasks~\cite{colloca2013support}, ~\cite{couceiro2017physiologically}, ~\cite{li2014machine}, ~\cite{li2013ventricular}.


% deep learning methods: non-recurrent
However, hand crafting descriptors and engineering features are very expensive, time-consuming and tedious process. Moreover, they demand the availability of expert knowledge. Convolutional Neural Networks (CNN) offer to automatize the features generation process without the need of an expert's supervision. This will produce more effective features, allow an end-to-end analysis on bigger data and better generalizes on unseen data. Deep CNNs have shown high performance on different computer vision and medical applications and in some cases they matched or even surpassed the human accuracy~\cite{lecun1995convolutional}, ~\cite{lecun2010convolutional}, ~\cite{krizhevsky2012imagenet}, ~\cite{lecun2015deep}. 
\end{comment}

Deep CNNs have also been adopted for ECG signal classification. 
%Kiranyaz et al.~\cite{kiranyaz2015real} have used 1-D CNN architectures for ECG signal classification. They trained a CNN for each patient with the goal of monitoring patient specific long-term ECG signal in real-time. In a more recent work, 
Rajpurkar et al.~\cite{rajpurkar2017cardiologist} proposed a 34-layer CNN for classifying 12 cardiological disorders by mapping the ECG signals to their corresponding rhythmic disorder classes. 
Andreotti et al.~\cite{andreotti2017comparing} used ResNets~\cite{he2016deep} for AF detection in ECG signals. The shortcut paths in ResNets help this convolutional architecture not to suffer from the gradient vanishing \cite{?}. %Furthermore, in this paper the QRST peaks were removed from the ECG signal and the residue was fed to the network. It, therefore, comprises of rather heavy pre-processing, which again makes it dependent on the presence of expert knowledge. 
An alternative to CNNs for feature learning and data representation and avoiding the feature hand crafting was proposed by~\cite{al2016deep}. In the representation block, they feed the raw ECG signals to a stacked denoising autoencoder and train it in an unsupervised manner. The result is then fed into a softmax regression layer.
%Yao et al.~\cite{yao2017atrial} process the ECG signals in a multi-scale manner using the multi-scale convolutional neural network (MCNN). The instantaneous heart rate sequences are fed to the network as input. They, furthermore, use an additional dataset in addition to their main training dataset and reported a performance boost, which shows the benefit of increasing the training dataset size.
Authors in~\cite{isin2017cardiac} use the famous AlexNet for feature extraction. They fed AlexNet with R-T segments, which are extracted from the ECG signals, and direct the result into a 2-layer feed-forward neural network for detecting normal beats, paced beats and Rbbb (Right Bundle Branch Blocks) beats.

% deep learning methods: Recurrent
%Limam et al.~\cite{limam2017atrial} got inspired by the popularity and good performance of recurrent neural networks (RNNs) on time-series data in sound and speech recognition fields. They developed an architecture with convolutional layers, followed by an RNN block, constructed using long short-term memory (LSTM) cells. They fed their network with both the ECG and heart rate as input. In order to immune their system to overfitting, they use dropout as the regularizer. As for the classification, they feed the output of the LSTM to a feed-forward network in one variant and to an SVM in another variant. They reported slightly better performance with the SVM classifier.
The work of Ziehlmann et al.~\cite{zihlmann2017convolutional} achieved one of the best classification performances in the PhysioNet 2017 challenge~\cite{clifford2017af}. They introduced deep architectures with both CNNs and RNNs blocks. They proposed two deep network variants: In the first architecture, they constructed a 24-layer CNN. In the second variant, which performed better, they fed the output of the aforementioned 24-layer CNN to an LSTM. The input to both networks were the log spectrogram of the ECG signals. Furthermore, an interesting distinction in their work was the three-phase training of the whole network. In the first training phase, they trained the CNN block of the network. Then, they attached the LSTM layer to the CNN blocks, froze the previously trained CNN and trained the resulting network. In the last training phase, they trained the whole network at once in order to fine-tune the weights in the CNN and LSTM blocks.
In a similar work, Chauhan et al.~\cite{chauhan2015anomaly} proposed to stack multiple LSTM layers for the task of cardiovascular anomaly detection from ECG signals.

%Another family of deep neural network architectures were used by Xiong et al.~\cite{xiong2017robust}. Their architecture consists of $16$ residual blocks, with a skip connection from the input to the output of each of these blocks. In their follow-up work~\cite{xiong2018ecg}, these $16$ residual blocks are then followed by a 3-layer LSTM network. They used batch normalization and dropout in all of the residual blocks in order to provide the network with some degree of regularization and immune their network to overfitting. 

% deep nets + handcrafted features
There are many works that attempted to combine the automatically learned features by CNNs and the hand-crafted features based on domain knowledge~\cite{hong2017encase}, ~\cite{teijeiro2018abductive}, ~\cite{zhang2017patient}, ~\cite{teijeiro2017arrhythmia}, ~\cite{vollmer2017can}. 
The most common hand crafted features in this group of attempts are Fourier transform and wavelet transform. 
Xia et al.~\cite{xia2018detecting} used short-term Fourier Transform (STFT) in one variant and Stationary Wavelet Transform (SWT) in the other variant as the input to their deep CNN. They reported that the network that was fed with SWT outperforms the one which was fed with STFT. They further claimed that both of their approaches outperforms the majority of the methods in the literature. 
Rubin et al.~\cite{rubin2017densely} took advantage of two four-level densely connected convolutional neural networks (DenseNets). They, however, applied a rather heavy pre-processing on the data prior to the network training phase. They first removed the baseline wander and then detected and segmented the QRS complexes from the ECG signals. Then, they detected the noisy signals using an average template matching correlation coefficient. The output was afterwards transformed to spectrogram using a moving window of size $75$ with $50\%$ overlap. The resulting signals were then fed to the DenseNet~\cite{huang2017densely}. In the post-processing phase, in the cases where the classifiers decision for noisy and Others classes were too close, they used AdaBoost-abstain for reinforcing the DenseNet's decision.
The later approaches, which combines heavy pre-/post-processing techniques with deep learning, do acquire respectable results. However, as it was previously noted, they are tedious and very domain-specific and require the presence of expert knowledge and human supervision. For instance, in the same application, changing the dataset can challenge these approaches as they hardly generalize in cross-domain fields.




==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************

